Cycle Analysis of Directed Acyclic Graphs

In this paper, we employ the decomposition of a directed network as an undirected graph plus its associated node metadata to characterise the cyclic structure found in directed networks by finding a Minimal Cycle Basis of the undirected graph and augment its components with direction information. We show that only four classes of directed cycles exist, and that they can be fully distinguished by the organisation and number of source-sink node pairs and their antichain structure. We are particularly interested in Directed Acyclic Graphs and introduce a set of metrics that characterise the Minimal Cycle Basis using the Directed Acyclic Graphs metadata information. In particular, we numerically show that Transitive Reduction stabilises the properties of Minimal Cycle Bases measured by the metrics we introduced while retaining key properties of the Directed Acyclic Graph. This makes the metrics consistent characterisation of Directed Acyclic Graphs and the systems they represent. We measure the characteristics of the Minimal Cycle Bases of four models of Transitively Reduced Directed Acyclic Graphs and show that the metrics introduced are able to distinguish the models and are sensitive to their generating mechanisms.

==> declarations.tex <==

\section*{Declarations}


\subsection*{Availability of data and materials}

Our code implementing these methods, the network data analysed during this study, and the datasets supporting the results discussed in this article are all available in a Github repository \url{https://github.com/vv2246/tr-dag-cycles}.


\subsection*{Competing interests}
  The authors declare that they have no competing interests.

\subsection*{Funding}

This work was funded by SoBigData++: European Integrated Infrastructure for Social Mining and Big Data Analytics (Grant agreement ID: 871042).

\subsection*{Author's contributions}

All authors developed the theoretical concepts and designed the experiments discussed in the paper. V.V.\ created the software used and performed the data analysis.
All authors wrote the manuscript, and reviewed the final version of the manuscript.
P.E.\ supervised the work.

